Prompt: Probability-Conserved Cross Section Biasing Monte Carlo Particle Transport System

An open source software package for simulating thermal neutron propagation in geometry is presented. In this system, neutron propagation can be treated by either the particle transport method or the ray-tracing method. Supported by an accurate backend scattering physics engine, this system is capable of reproducing neutron scattering experiments in complex geometries and is expected to be used in the areas of instrument characterisation, optimisation and data analysis. In this paper, the relevant theories are briefly introduced. The simulation flow and the user input syntax to control it are provided in detail. Five benchmarking simulations, focusing on different aspects of simulation and scattering techniques, are given to demonstrate the applications of this simulation system. They include an idealised total scattering instrument, a monochromatic powder diffractometer, a neutron guide, a chopper and an imaging setup for complex geometries. Simulated results are benchmarked against experimental data or well-established software packages when appropriate. Good agreements are observed.

==> src/performance.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{{single_thread_performance}.png}
\caption{The performance of Prompt run in a single thread}\label{fSinThr}
\end{figure}

Prompt was initially designed as a single thread program,  Fig.~\ref{fSinThr} shows the time spent versus neutrons count run at a server with Intel Xeon Gold 5218 CPUs. It is clear that calculation will be completed in less than 1 minute when neutrons are less than \num{1e5}. However, with more particles, the time will increase linearly. With \num{1e9} neutrons, the calculation almost took 32.8 hours (118117 seconds).

In order to reduce the time when track a mount of particles, a Spark cluster is employed to enable the parallel computing of Prompt. The details of the Spark cluster is shown in Table.~\ref{tableSpark}. This cluster composes of 5 nodes, with total 496 CPU cores. All nodes with the same Spark, Java Development Kit (JDK), and Operating System (OS) deployed.

\begin{table}
	\centering                       
	\caption{Details of Spark Cluster}     
	\label{tableSpark} 
	
    \begin{tabular}{p{8em}p{24em}} 
    \toprule
    Item & Information   \\ 
    
    \midrule
    \texttt{Spark Version} & spark-3.2.1-bin-hadoop3.2-scala2.13.\\
    \texttt{Deploy Mode} & Standalone.\\ 
    \texttt{Java Version} & OpenJDK 1.8.0\_332 (Temurin).\\ 
    \texttt{OS} & Ubuntu 20.04.4 LTS.\\ 
    \texttt{Node 1} & 64 cores (2 Intel(R) Xeon(R) Gold 5218 CPUs).\\
    \texttt{Node 2} & 64 cores (2 Intel(R) Xeon(R) Gold 5218 CPUs).\\ 
    \texttt{Node 3} & 96 cores (2 Intel(R) Xeon(R) Gold 6248R CPUs).\\
    \texttt{Node 4} & 96 cores (2 Intel(R) Xeon(R) Gold 6248R CPUs).\\
    \texttt{Node 5} & 176 cores (4 Intel(R) Xeon(R) Gold 6238 CPUs).\\
    
    \bottomrule
    \end{tabular}
\end{table}

The time spent versus CPU cores with \num{1e9} neutrons run in the Spark cluster is shown in Fig.~\ref{fSpark1e9}. With 10 cores, it took 210 minutes, while with 450 cores, 10 minutes, that's 20x fast. Also note, the performance improved much obviously when CPU cores less than 100. With more cores, the performance improvement slowed down. So in practice, there is a compromise between time and cores.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{{spark_performance_1e9_neutrons}.png}
\caption{The performance of Prompt run in a Spark cluster (\num{1e9} neutrons)}\label{fSpark1e9}
\end{figure}

As a complement of the evaluation, the time spent versus CPU cores in the Spark cluster when simulating 1 neutrons has also been investigated. Shown in Fig.~\ref{fSpark1}. It took 3 seconds with 1 core, while 7 seconds with 450 cores. It is shown that it has some intrinsic cost when run in Spark. With 1 neutron, the more cores used, the more time spent. The plot profile is of the step form, due to the measurement temporal precision of 1 second.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{{spark_performance_1_neutron}.png}
\caption{The performance of Prompt run in a Spark cluster (\num{1} neutrons)}\label{fSpark1}
\end{figure}

It is 0.06 second when running in the single threading mode with 1 neutron, while comparing to 3 seconds running in the Spark cluster with 1 core. Fig.~\ref{fSinThr} also shows it is about 12 seconds when simulating \num{1e5} neutrons in single threading mode. So how to choose the mode \texttt{Prompt} run, it depends.
